Corruption-Robust Offline Two-Player Zero-Sum Markov Games

We study data corruption robustness in offline two-player zero-sum Markov games. Given a dataset of realized trajectories of two players, an adversary is allowed to modify an $\epsilon$-fraction of it. The learner's goal is to identify an approximate Nash Equilibrium policy pair from the corrupted data. We consider this problem in linear Markov games under different degrees of data coverage and corruption. We start by providing an information-theoretic lower bound on the suboptimality gap of any learner. Next, we propose robust versions of the Pessimistic Minimax Value Iteration algorithm, both under coverage on the corrupted data and under coverage only on the clean data, and show that they achieve (near)-optimal suboptimality gap bounds with respect to $\epsilon$. We note that we are the first to provide such a characterization of the problem of learning approximate Nash Equilibrium policies in offline two-player zero-sum Markov games under data corruption.

==> main_paper/checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
% Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% \textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes] We provide theoretical analyses on the convergence of our proposed methods.
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Not Applicable]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes] All proofs are given in the Appendix.
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable] 
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not Applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

==> main_paper/old.tex <==
%Describe briefly PMVI 
%Describe briefly SCRAM



% ---------------- OLD ---------------- \\

%
% To answer this question, we build upon a recent offline MARL approach -- Pessimistic Minimax Value Iteration (PMVI) \citep{zhong2022pessimistic} -- designed for corruption-free settings. In a nutshell, PMVI combines backward induction  with the pessimism principle to learn an approximate NE policy pair in \emph{linear Markov games} (see Definition~\ref{asmp_linearity}). 
%and we combine it with recently proposed robust estimation techniques~\cite{}.
%
% PMVI enjoys a near-optimal bound on the suboptimality under the {\em low relative uncertainty} (LRU) coverage assumption (see Assumption \ref{asm:low_relative_uncertainty}).
%Compared to standard coverage assumptions, LRU is  a weaker condition than uniform coverage assumption, and as we show in this paper, comparable to unilateral coverage assumption. 
% Inspired by recent works in corruption-robust single-agent offline RL \citep{zhang2022corruption}, we robustify PMVI with different robust estimation techniques as our main contribution.
%
%\subsection{Our contributions}
% More concretely, we analyze the problem along the following dimensions: (i) degree of corruption; (ii) coverage assumption (LRU or \emph{Uniform} $\Sigma$); (iii) game setting (\emph{linear} or \emph{tabular}). In particular, we consider two degrees of corruption depending on if the corruption 
% is limited to manipulating rewards / next states in the data (referred to as \emph{clean covariates}) or if the corruption is unrestricted (\emph{corrupted covariates}).
% We propose different corruption-robust variants of PMVI along these dimensions and provide a rigorous analysis of their optimality bounds. 


% we consider the following three robust estimation approaches for different degrees of corruption: (i) Spectrally Regularized Alternating Minimization (SCRAM) \citep{chen2022online} for weak corruption, (ii) Robust Least Squares (RLS) \citep{zhang2022corruption} and Filtering \citep{diakonikolas2017being} for strong corruption. 
% We consider both tabular and linear Markov game settings, under LRU, which is the weakest coverage assumption necessary to solve the problem, and the more generous uniform $\Sigma$-coverage assumption, which we introduce in this work. In both cases, we provide near-optimal bounds on the suboptimality, both in terms of estimation error and corruption error. Our main contributions can be summarized as follows. For a detailed illustration of our results, see Table \ref{tab:summary}.

% We prove that it incurs $O(H^2d\epsilon + H^2K^{-1/2}d^{3/2})$ bound on the suboptimality gap, under the Low Relative Uncertainty (LRU) assumption and a corruption model that corrupts an $\epsilon$-fraction of the rewards and the next states in the offline data. We note that, under no corruption, we recover the state-of-the-art (SOTA) bounds of \cite{zhong2022pessimistic}, while there is a $\sqrt{\epsilon}$ factor of improvement in the corruption error compared to the single agent SOTA \citep{zhang2022corruption}, \textit{thus matching the information-theoretic lower bound} in terms of $\epsilon$. This is arguably due to the tight analysis accompanied by the efficiency of SCRAM. 
%
% \item \textbf{LRU and corrupted covariates.} Combining the two weakest assumptions, we propose F-PMVI, which uses the Filtering oracle \citep{diakonikolas2017being} as a robust estimator for the tabular setting, and show that it achieves a near-optimal bound on the suboptimality gap with high probability, under \textit{arbitrary corruption and LRU coverage} assumptions.
%
% \item \textbf{Impossibility result.} Finally, we show that convergence to Nash equilibria, without knowledge of $\epsilon$ and uniform coverage, is impossible in the offline two-player zero-sum setting, extending a similar result for single-player settings \citep{zhang2022corruption}.



%Given such intricacies of multi-agent settings, corruption robustness in offline MARL is much less understood.

% due to the following challenges
%Moreover, the coverage assumptions of data-collecting policies required by algorithms are a lot more intricate in multi-agent settings.

%The agent has to rely on the data-collecting policy, so adequate coverage assumptions are usually necessary. Furthermore, optimality in such problems is equivalent to learning Nash Equilibria (NE), making algorithmic design in such systems more complicated. 




% The aforementioned challenges have recently been addressed for various instances of the MARL framework, in linear and tabular settings, where algorithms such as PMVI enjoy near-optimal suboptimality gap bounds in clean environments.

% The growing presence of abundant data has facilitated the rise of offline Reinforcement Learning (RL). While online experimentation and dynamic interaction with the environment allow traditional online RL to capture key properties of real-life scenarios, in applications such as autonomous driving \citep{pan2017agile}, or healthcare \citep{wang2018supervised}, such experimentation becomes extremely expensive or dangerous. Therefore, the utilization of available historical data becomes paramount. Many of these applications, however, can be better captured by the mathematical formalism of Multi-agent RL (MARL): autonomous drivers have to account for the presence of multiple agents; mental healthcare professionals have to account for the intricacies of patient interactions for efficient care coordination \citep{kalton2016multi}, thus making Offline MARL an important area of research. 

% However, offline MARL comes with additional challenges. Here, a dynamic exploration of the environment is impossible, and thus, the principle of \textit{pessimism in the face of uncertainty} seems to be the primary paradigm of learning. Moreover, the agent has to rely on the data-collecting policy, so adequate coverage assumptions are usually necessary. Last, but not least, optimality in such problems is equivalent to learning Nash Equilibria (NE), making algorithmic design in such systems more complicated. The aforementioned challenges have recently been addressed for various instances of the MARL framework, in linear and tabular settings, where algorithms such as PMVI enjoy near-optimal suboptimality gap bounds in clean environments.

% Unfortunately, it is rarely the case in practical scenarios that the data is sampled from a latent distribution with "nice" properties. Adversarial attacks in ML are becoming increasingly present in modern systems: adversarial stickers can jeopardize the performance of autonomous vehicles \citep{eykholt2018robust}, while fake reviews can manipulate the behavior of recommendation systems. These threats are also extended to offline MARL. The threat is even more serious in this setting since data corruption might render a notion of equilibrium unintelligible.  While this problem has been studied in the single-player setting, data corruption in Markov games has been unexplored. Motivated by these observations, we initiate the study of robustness to arbitrary data corruption in Offline Markov games. The goal of this paper is to answer the following question:

% \textit{Can we design algorithms that approximately solve offline two-player zero-sum Markov games under the presence of data corruption?}

% To answer this question, we consider both tabular and linear Markov game settings, under Low Relative Uncertainty (LRU), which is the weakest coverage assumption necessary to solve the problem and the more generous uniform $\Sigma$-coverage assumption. In both cases, we are able to show near-optimal bounds on the suboptimality gap, both in terms of estimation error and corruption error. Our main contributions can be summarized as follows. For a detailed illustration of our results, see Table \ref{tab:summary}.


% Since Offline MARL methods rely on clean data samples, the study of the statistical robustness of Offline MARL methods under data corruption becomes highly important. With that being said, we initiate the study of the statistical robustness of Offline MARL, by considering two-player zero-sum Markov games, in both linear and tabular settings, under different assumptions on the data-collecting policy, and different corruption models. 


% Offline Reinforcement Learning (RL) has become an important  topic in recent years \citep{levine2020offline, lange2012batch, agarwal2020optimistic}. This increasing interest is arguably due to its appealing property of utilizing offline historical data and, thus, avoiding expensive online experimentation. This property proves extremely useful in applications such as auto-driving \citep{pan2017agile} and healthcare \citep{wang2018supervised}, where, apart from being expensive, in some cases, data collection is not even possible \citep{fu2020d4rl}. The study of theoretical properties of Offline RL has not been left behind \citep{jin2021pessimism, xie2021bellman, rashidinejad2021bridging, uehara2021pessimistic, zanette2021provable}. Since the online exploration of the environment is lacking, being optimistic in such a scenario "might hurt". Indeed, the principle of \textit{pessimism in the face of uncertainty} seems to be critical for learning provably efficient strategies in this setting. Another key challenge of computing optimal strategies solely based on collected data is the distributional shift between the behavioral policy and the optimal policy. Thus, if there is to be any hope of learning, additional assumptions on the data-collecting strategy are necessary. 

% An important extension of Offline RL is Offline Multi-agent Reinforcement Learning (MARL) \citep{yang2021believe, cui2022provably, jiang2021offline, busoniu2008comprehensive}, where the collected data is comprised of multiple agents' trajectories, that simultaneously affect transition dynamics of the environment. In this setting, learning faces an additional challenge: the principle of optimality is not reward maximization, but convergence to equilibria, preferred by all agents in the system. Recent works \citep{zhong2022pessimistic, cui2022offline} have considered integrating the pessimism principle into \textit{offline two-player zero-sum Markov games} (MG), which are the simplest examples of Markov games. The natural extension of Pessimistic Value Iteration \citep{liu2020provably, buckman2020importance} into the offline two-player zero-sum MG setting is Pessimistic Minimax Value Iteration (PMVI) which is provably efficient \citep{zhong2022pessimistic}. The main distinguishing characteristic of PMVI is that it behaves pessimistically with respect to the $Q$-value estimates of both players, while it assumes that the underlying MG is linear \citep{jin2020provably}. 

% RL with linear function approximation has gained quite some focus lately \citep{jin2020provably, melo2007q}. The nice structure that this assumption implies on the underlying MDP facilitates theoretical understanding of such objects. Furthermore, it makes the estimation problem in examples with extremely large state spaces possible. In the Offline (MA)RL setting, the problem reduces to linear regression on observations of the $Q$-values. The aforementioned versions of Value Iteration for two-player zero-sum Markov games rely on such an assumption. 

% All the aforementioned scenarios have already been considered under standard statistical assumptions on the data. However, it is not always the case that the dataset is sampled from a latent distribution with "nice" properties. One of the main security threats to modern Machine Learning systems is data corruption: Twitter chatbots were adversarially manipulated into making inappropriate comments \citep{neff2016talking}; autonomous vehicles can be misled by adversarially modified stickers \citep{eykholt2018robust}; recommendation systems can be manipulated by fake reviews. Since Offline MARL methods rely on clean data samples, the study of the statistical robustness of Offline MARL methods under data corruption becomes highly important. With that being said, we initiate the study of the statistical robustness of Offline MARL, by considering two-player zero-sum Markov games, in both linear and tabular settings, under different assumptions on the data-collecting policy, and different corruption models. 


%%%%%%%%%%  LINEAR   SETTING    %%%%%%%%%%%%%%%%%%%%%%



% We start by stating the linearity assumption for Markov games, standard in the literature \citep{xie2020learning}.
% \begin{assumption}[Linearity of MG]\label{asmp_linearity}
%  For each $(s,a,b)\in \mathcal{S}\times \mathcal{A}\times \mathcal{B}$ we have
% \begin{align*}
%     r_h(s,a,b) & = \phi(s,a,b)^\top \theta_h + \zeta \;\; \text{and} \\
%     p_h(\cdot |s,a,b) & = \phi(s,a,b)^\top \mu_h(\cdot)~,
% \end{align*}
% where $\phi : \mathcal{S}\times \mathcal{A} \times \mathcal{B} \rightarrow \mathbb{R}^d$ is a known feature map, $\theta_h \in \mathbb{R}^d$ is an unknown vector, $\zeta$ is zero-mean $\gamma^2$-subGaussian noise and $\mu_h=(\mu^{(i)}_h)_{i \in [d]}$ is a vector of $d$ unknown signed measures on $\mathcal{S}$. We assume that $\norm{\phi(\cdot,\cdot,\cdot)}_2 \leq 1$, $\norm{\theta_h}_2\leq \sqrt{d}$ and $\norm{\mu_h(\mathcal{S})}_2\leq\sqrt{d}$, for all $h\in [H]$. 
% \end{assumption}

% \begin{align*}
%     Q^{\pi,\nu}_h(s,a,b) & = \mathbb{E}[r_h(s,a,b)] + p_h(\cdot |s,a,b)^\top V^{\pi,\nu}_{h+1} \\
%                          & = \phi(s,a,b)^\top \theta_h + (\phi(s,a,b)^\top \mu_h)^\top V^{\pi,\nu}_{h+1} \\
%                          & = (\theta_h + \mu_h^\top V^{\pi,\nu}_{h+1})^\top \phi(s,a,b) \\
%                          & := \phi(s,a,b)^\top \omega^*_h~.
% \end{align*}

% Formally, at each time step $h\in[H]$, it maintains
% \begin{align*}
%     \underline{Q}(\cdot,\cdot,\cdot) & = \Pi_{H-h+1}\left( \phi(\cdot,\cdot,\cdot)^\top \underline{\omega}_h - \Gamma_h(\cdot,\cdot,\cdot) \right), \\ % \label{eq:q_matrix_1} \\
%     \overline{Q}(\cdot,\cdot,\cdot) & = \Pi_{H-h+1}\left( \phi(\cdot,\cdot,\cdot)^\top \overline{\omega}_h + \Gamma_h(\cdot,\cdot,\cdot) \right)~,% \label{eq:q_matrix_2}
% \end{align*}
% where 
% \begin{align*}
%     \Gamma_h(s,a,b) =\left(\sqrt{K} \mathcal{E} + 2H\sqrt{d} \right) \norm{\phi(s,a,b)}_{\Lambda_h^{-1}}~.
% \end{align*}
% Here 
% \begin{align*}
%     \Lambda_h = \sum^K_{\tau=1}\phi(s^\tau_h,a^\tau_h,b^\tau_h)\phi (s^\tau_h,a^\tau_h,b^\tau_h)^\top + I
% \end{align*}
% denotes the regularized samples covariance matrix, and $\mathcal{E}$ denotes\footnote{For a detailed definition, see  the Appendix.} the upper bound in \eqref{eq:scram_approximate}. 
%


% \begin{align*}
%     (\widehat{\pi}_h,\nu'_h) & \leftarrow NE(\underline{Q}(\cdot,\cdot,\cdot) ) \\ % \label{eq:ne_strategy_estimates_1}\\
%     (\pi',\widehat{\nu}_h) & \leftarrow NE(\overline{Q}(\cdot,\cdot,\cdot) )~.% \label{eq:ne_strategy_estimates_2}
% \end{align*}

% \begin{align*}
%     \underline{V}_h(\cdot) & = \mathbb{E}_{a\sim \widehat{\pi}(\cdot |\cdot),b\sim \nu'(\cdot |\cdot)}[\underline{Q}_h(\cdot,a,b)] \\ %\label{eq:estimated_values_1}\\
%     \overline{V}_h(\cdot) & = \mathbb{E}_{a\sim \pi'(\cdot |\cdot),b\sim \widehat{\nu}(\cdot |\cdot)}[\overline{Q}_h(\cdot,a,b)] %\label{eq:estimated_values_2}
% \end{align*}

% \begin{rem}
%     Note that R-PMVI does not use a bonus term. Thus, it does not require any knowledge of $\epsilon$, apart from the RLS oracle. The bounds, however, hold the same. This is due to the linear assumption and the robust least squares estimator and the style of analysis.
% \end{rem}


% However, the presence of corruption in the dataset necessitates the usage of robust estimators. In single-player offline RL, the authors of \citep{ZCZS22} use a Robust Least Squares Oracle that returns an estimator which incurs $\tilde{O}(\epsilon)$ least square error. However, such an estimator requires Assumption \ref{asn:uniform-phi-coverage} to hold. 

% Note that the assumption above requires $\mathbb{E}_\nu[xx^\top]\geq \xi$, which, as shown in Lemma \ref{lem_strong_assumption}, is stronger than the uniform coverage assumption when we let $x_i=\phi(s^i_h,a^i_h,b^i_h)$, for some $h\in[H]$.


% For the robustness problem in single agent offline RL, the authors of \citep{zhang2022corruption} utilize a Robust Least Squares (RLS) estimator which requires Assumption \ref{asn:uniform-phi-coverage} to hold. However, for the two-player zero-sum MG setting, only unilateral coverage is required to compute an approximate NE pair from offline data \citep{zhong2022pessimistic}. Thus, the question arises whether we can recover "good enough" estimates in the two-player zero-sum setting without the need for such a strong assumption. 

%
% First, note that, for each set $D_h$, the level of corruption $\epsilon_h$ is at most $\epsilon$, since $\sum^H_{h=1}\epsilon_hK \leq \epsilon KH$. Thus, we can call SCRAM with different batches of the dataset with the same parameter $\epsilon$. Then, for each time step $h=H, H-1,\ldots,1$, we obtain
% \begin{align*}
%     \underline{\omega}_h & \leftarrow SCRAM \Bigl( \{ \phi(s^\tau_h,a^\tau_h,b^\tau_h), r^\tau_h + \underline{V}_{h+1}(s^\tau_{h+1}\}^K_{\tau=1} \Bigr) \\
%     \overline{\omega}_h & \leftarrow SCRAM \Bigl( \{ \phi(s^\tau_h,a^\tau_h,b^\tau_h), r^\tau_h + \overline{V}_{h+1}(s^\tau_{h+1}\}^K_{\tau=1} \Bigr)
% \end{align*}
% Once we have estimates of the true weights, the algorithm proceeds to construct estimates of the $Q$-values for both players. Formally, at each time step $h\in[H]$, it maintains
% \begin{align*}
%     \underline{Q}(\cdot,\cdot,\cdot) & = \Pi_{H-h+1}\left( \phi(\cdot,\cdot,\cdot)^\top \underline{\omega}_h - \Gamma_h(\cdot,\cdot,\cdot) \right), \\ % \label{eq:q_matrix_1} \\
%     \overline{Q}(\cdot,\cdot,\cdot) & = \Pi_{H-h+1}\left( \phi(\cdot,\cdot,\cdot)^\top \overline{\omega}_h + \Gamma_h(\cdot,\cdot,\cdot) \right)~,% \label{eq:q_matrix_2}
% \end{align*}
% where 
%
% Next, we solve the matrix games with payoffs $\underline{Q}(\cdot,\cdot,\cdot) $ and $\overline{Q}(\cdot,\cdot,\cdot) $ and obtain
% \begin{align*}
%     (\widehat{\pi}_h,\nu'_h) & \leftarrow NE(\underline{Q}(\cdot,\cdot,\cdot) ) \\ % \label{eq:ne_strategy_estimates_1}\\
%     (\pi',\widehat{\nu}_h) & \leftarrow NE(\overline{Q}(\cdot,\cdot,\cdot) )~.% \label{eq:ne_strategy_estimates_2}
% \end{align*}
% Finally, the value functions are estimated as
% \begin{align*}
%     \underline{V}_h(\cdot) & = \mathbb{E}_{a\sim \widehat{\pi}(\cdot |\cdot),b\sim \nu'(\cdot |\cdot)}[\underline{Q}_h(\cdot,a,b)] \\ %\label{eq:estimated_values_1}\\
%     \overline{V}_h(\cdot) & = \mathbb{E}_{a\sim \pi'(\cdot |\cdot),b\sim \widehat{\nu}(\cdot |\cdot)}[\overline{Q}_h(\cdot,a,b)] %\label{eq:estimated_values_2}
% \end{align*}
%
% After $H$ steps, the algorithm terminates and outputs the estimated pairs of strategies $(\widehat{\pi},\widehat{\nu})$. We give the pseudocode of our proposed method in the Appendix. 
%

%
% \begin{rem}
%     Theorem \ref{thm:linear_case} holds under Assumption \ref{asm:low_relative_uncertainty}, which requires the covariates to be clean. However, Assumption \ref{asn:unilateral-coverage} is a weaker assumption than both Assumptions \ref{asn:uniform-coverage} and \ref{asn:uniform-phi-coverage}. Note that S-PMVI is able to incur upper bounds on the gap that have optimal dependence on $\epsilon$. If we want to get similar results under weaker assumptions on the corruption model, there is a trade-off, in the sense that we need stronger assumptions on the data coverage.
% \end{rem}


% in certain examples (e.g. when $\Lambda_h$ has all eigenvalues equal to $K-1$ and the left-hand side matrix has the first one equal to $1+c_1Kd$ and all others $1$, $c_1$ can be as low as $1/d$


%%%%%%%%%    TABLE     %%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table*}[!t]
% \renewcommand{\arraystretch}{1}
%     \centering
%     % \footnotesize
%     \scalebox{0.9}
% {
% \begin{tabular}{l c c l c l}\toprule
%         Coverage & & \multicolumn{2}{c}{Clean Covariates} & \multicolumn{2}{c}{Corrupted Covariates}\\
%         \midrule
%         \multirow{2}{4.5em}{LRU}
%             & Tabular & \a & [Cor. \ref{cor:tabular_scram}] & \e & [Thm. \ref{thm:filtering}] \\
%             & Linear & \b & [Thm. \ref{thm:linear_case}] & $-$ & \\
%         \cmidrule{2-6}
%         \multirow{2}{4.5em}{Uniform $\Sigma$}
%             & Tabular & \c & [Cor. \ref{cor:tabular_rls}] & \c & [Cor. \ref{cor:tabular_rls}] \\
%             & Linear & \d & [Thm. \ref{thm:linear_uniform_coverage}] & \d  & [Thm. \ref{thm:linear_uniform_coverage}]\\
%          \bottomrule
% \end{tabular}
% }
% %\end{adjustbox}
% \vspace{0.1in}
% \caption{Summary of our results for the tabular and linear settings, under Low Relative Uncertainty and uniform $\Sigma$-coverage assumptions (see Assumptions \ref{asn:unilateral-coverage} and \ref{asn:uniform-phi-coverage} for definitions), and different corruption levels of the feature covariance matrix. Here $\epsilon$ denotes the corruption level and $f(x)$ denotes a polynomial function of $x$.  We have omitted linear dependence on noise variance $\gamma^2$ of the rewards for ease of presentation. We point the reader to the relevant results for a detailed description. We note that the universal lower bound for the offline two-player zero-sum MG setting is $\Omega (Hd\epsilon)$ (or $\Omega (HSAB\epsilon)$ for tabular MGs), given in Theorem \ref{thm:lower_bound}. }
% \label{tab:summary}
% \vspace{-0.2cm}
% \end{table*}


%
% \textit{Proof sketch.} Using a variant of Cauchy-Schwarz, we upper-bound the Bellman error in terms of the feature norms which depend on the corrupted covariance matrix. Since LRU holds only on the clean data, we decompose the inverse covariance matrix using a version of the Woodbury inversion identity and separate the error into the one coming from the clean data, which is immediately bounded as in the clean case, and one coming from corrupted samples, which we deal with by using matrix analysis properties. 
%



%%%%%%%%%%%%%     RELATED WORK   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Due to its appealing properties, offline RL, also known as batch RL, has been gaining increasing attention recently \citep{levine2020offline, lange2012batch, agarwal2020optimistic}. The two main categories of approach  (regularized policy-based and pessimistic value-based) show impressive empirical success. On the theoretical front, the works are worth mentioning, all of which share the common view that pessimism is the key to addressing the lack of exploration in this setting. 

% While 

% offline MARL  has also gained in popularity in the past few years, with the works of \cite{yang2021believe, pan2022plan}. We draw attention to a special case of this paradigm, namely, the problem of data corruption in Offline two-player zero-sum games. 

% Unfortunately, the robustness to adversarial attacks in Markov games  has been unexplored. We study the robustness problem in Offline two-player zero-sum Markov games \citep{zhong2022pessimistic, cui2022provably}. The offline problem in Markov games has also been recently studied in the harder multi-player general-sum setting \citep{cui2022provably}. We hope this work motivates the further study of robustness in this setting. 

==> main_paper/tabular_setting.tex <==
\section{RESULTS FOR TABULAR MARKOV GAMES}\label{sec:tabular_setting}

In this section, we will consider both LRU and $\Sigma$-coverage assumptions. We start by discussing the latter, as it will be a corollary of the linear setting under the same assumptions. Then, we move on to the weaker LRU assumption, while also considering an arbitrary corruption model. 

\subsection{Uniform $\Sigma$-coverage and Corrupted Covariates}

The tabular MGs can be seen as a special case of linear MGs, where the dimension $d$ is just $SAB$ and the features of state-action tuples can be thought of as $SAB-$dimensional one-hot encoding vectors, where the $i$th component is $1$ if and only if it corresponds to $(s,a,b)$. It is always possible to use any of the robust estimators that were mentioned in previous sections in the tabular setting. In that case, the bounds on the suboptimality gap would be imported from previous results, by substituting $d$ with $SAB$, as we formally state below.
\begin{cor}\label{cor:tabular_rls}
    Given a tabular Markov game $\mathcal{G}=(\mathcal{S},\mathcal{A},\mathcal{B},P,r,H)$, suppose offline data $D$  is $\Sigma$-covered. Moreover, given $\epsilon>0$, assume that $\epsilon$-fraction of $D$ is arbitrarily corrupted by an adversary. Then, with probability at least $1-\delta$, R-PMVI that uses features defined as one-hot encoding vectors, incurs
    \begin{equation*}
         \optgap(\widehat{\pi},\widehat{\nu}) \leq O \left( \sqrt{\frac{H^2poly(SAB)}{K}} + H^2(SAB)\epsilon \right)~.
    \end{equation*}
\end{cor}

\subsection{LRU Coverage and Corrupted Covariates}

First, we state a result for clean covariates, which is an immediate corollary of Theorem \ref{thm:linear_case}.
\begin{cor}\label{cor:tabular_scram}
     Given a tabular Markov game $\mathcal{G}=(\mathcal{S},\mathcal{A},\mathcal{B},P,r,H)$, suppose Assumption \ref{asm:low_relative_uncertainty} (with constant $c_1$) holds. Moreover, given $\epsilon>0$, assume that $\epsilon$-fraction of rewards and next states of the data is corrupted by an adversary, i.e. the state-action tuples remain clean. Then, with probability at least $1-\delta$,  R-PMVI that uses features defined as one-hot encoding vectors, incurs
    \begin{equation*}
         \optgap (\widehat{\pi},\widehat{\nu},s)  \leq O\left( \frac{1}{\sqrt{c_1}}H^2\sqrt{SAB}\epsilon + \frac{H^2SAB}{\sqrt{c_1K}}\right)~.
    \end{equation*}
\end{cor}

However, the tabular setting is simpler in structure than the linear one. The rewards and transitions can always be estimated by sample averages, instead of using robust least square estimators. Also,  the covariance matrix of the observations here becomes diagonal, and thus, simpler to handle.  Thus, we ask the question: Can we design a robust version of PMVI for tabular MGs, that uses an arbitrarily corrupted dataset, while it only needs LRU coverage?

We answer this question in the affirmative. To that end, we apply the filtering technique \citep{diakonikolas2017being} on the $SAB$-dimensional reward vectors and $S^2AB$-dimensional transition vectors. The following result gives upper bounds on the error of the estimation up to logarithmic factors, for distributions with bounded moments. 

\begin{thm}[\cite{diakonikolas2017being}]\label{thm:filtering}
    Let $P$ be a distribution in $\mathbb{R}^d$ with unknown mean vector $\mu^P$ and unknown covariance matrix $\Sigma_P \preceq \sigma^2 I$. Let $S$ be an $\epsilon$-corrupted set of samples from $P$ of size $O ((d/\epsilon)\log (d/\delta))$. There exists an efficient algorithm that, on input $S$ and $\epsilon >0$, with probability at least $1-\delta$, outputs $\widehat{\mu}$ with $\norm{\widehat{\mu} - \mu^P}_2 \leq O\left( \sigma\sqrt{\epsilon} \right).$

\end{thm}

% Note that, since the feature matrix $\Phi$ is the identity matrix, for each $h\in[H]$, the sample covariance matrix becomes
% \begin{equation*}
%     \frac{1}{K}\sum^K_{\tau=1}\phi(s^\tau_h,s^\tau_h,b^\tau_h) \phi (s^\tau_h,s^\tau_h,b^\tau_h)^\top = \Phi^\top  \widehat{D}_h \Phi =  \widehat{D}_h~,
% \end{equation*}
% where $ \widehat{D}_h$ is the diagonal $SAB\times SAB$-dimensional matrix with entries as frequencies of occurrences of each $(s,a,b)$. 
Now, given $\tau \in [K]$, denote by $R^\tau_h$ the $SAB$-dimensional vector
\begin{equation*}
    R^\tau_h(s,a,b)=
    \begin{cases}
        r_h(s^\tau_h,a^\tau_h,b^\tau_h) & \; \text{if} \; (s^\tau_h,a^\tau_h,b^\tau_h) = (s,a,b) \\
        0 & \; \text{otherwise}
    \end{cases}
\end{equation*}
% \begin{equation}\label{eq:r_estimates_tabular}
%     \widehat{r}_h(s,a,b)=\frac{1}{K}\sum^K_{\tau=1}r^\tau_h\mathbf{1}\{ (s^\tau_h,a^\tau_h,b^\tau_h) = (s,a,b)\}~,
% \end{equation}
as a sample of the random vector $R_h$ with mean $\mu(r_h)$. Furthermore, let $P^\tau_h$ denote the $S^2AB$-dimensional vector with entries 
\begin{equation*}%\label{eq:p_estimates_tabular}
     P^\tau_h(s,a,b,s') = \frac{\mathbf{1}\{ (s^\tau_h,a^\tau_h,b^\tau_h,s^\tau_{h+1})=(s,a,b,s')\}}{\frac{1}{K}\sum^K_{\tau=1}\mathbf{1}\{ (s^\tau_h,a^\tau_h,b^\tau_h)=(s,a,b)\} }~,
\end{equation*}
being a realization of the random vector $P_h$ with mean $p_h$. Now let $N_h$ denote the $S^2AB\times S^2AB$-dimensional diagonal matrix with entries $1/n(s,a,b,s')$, where
\begin{align*}
    n_h(s,a,b,s')& =n(s,a,b,s'') \\ & = 1 \vee \sum^K_{\tau=1}\mathbf{1}\{ (s^\tau_h,a^\tau_h,b^\tau_h)=(s,a,b)\}~,
\end{align*}
for all $(s,a,b)$. Then, note that the following relations hold.
\begin{equation*}
    Cov(R_h) = \gamma^2 I \;\; \text{and} \;\; Cov(P_h) = N_h \preceq I~.
\end{equation*}
Also, recall that we assume $D_h$ subsets are independent across $h\in[H]$. Thus, we have proven the following corollary. 
\begin{cor}\label{cor:filtering_pmvi}
    Let $K = \Theta ((S^2AB)/\epsilon)\log (S^2ABH/\delta))$. There exists an algorithm that, on input $D_h$ and $\epsilon$, with probability $1 - \delta$, outputs $\widehat{r}_h$ and $\widehat{p}_h$ that satisfy
    \begin{align*}
        \norm{\widehat{r}_h - \mu(r_h)}_2 & \leq \sqrt{\epsilon}\gamma \;\; \text{and} \;\;
        \norm{\widehat{p}_h - p_h}_2  \leq \sqrt{\epsilon}~,
    \end{align*}
    for all $h\in[H]$.
\end{cor}
Assuming access to the Filtering subroutine, we propose Filtering-PMVI (F-PMVI), which uses the Filtering oracle as a robust estimator of sample means of rewards and transition probabilities, and then follows the procedure of PMVI to compute the estimated NE strategies $(\widehat{\pi},\widehat{\nu})$ over $H$ time steps. 
The difference between F-PMVI from S-PMVI, besides the different robust oracle that it uses, is the estimation of the $Q$-values. Since we are in the tabular setting, for every $h\in[H]$, F-PMVI sets\footnote{We omit dependence on $(s,a,b)$ for brevity of notation.}
\begin{align}
    \underline{Q}_h & = \Pi_{H-h+1}\left( \widehat{r}_h + \widehat{p}_h(\cdot)^\top \underline{V}_{h+1}(\cdot) - \Gamma\right) \label{eq:tabular_values_estimates_1}~, \\
     \overline{Q}_h & = \Pi_{H-h+1}\left( \widehat{r}_h + \widehat{p}_h(\cdot)^\top \overline{V}_{h+1}(\cdot) + \Gamma \right)\label{eq:tabular_values_estimates_2}~, 
\end{align}
where 
\begin{equation}\label{eq:filtering_bonus}
    \Gamma (s,a,b) = O( (H\sqrt{S} + \gamma ) \sqrt{\epsilon} )
\end{equation}
is the bonus term. The rest of the algorithm follows the same logic as S-PMVI and R-PMVI. The pseudocode is given in the Appendix. We proceed with the main result of this section, which provides a high-probability upper bound on the suboptimality gap of the strategies returned by F-PMVI.

\begin{thm}\label{thm:tabular_filtering}
    Let $\mathcal{G}=(\mathcal{S},\mathcal{A},\mathcal{B},P,r,H)$ be a tabular MG. Assume offline data $D$ is $\epsilon$-corrupted arbitrarily by an adversary and that it satisfies Assumption \ref{asn:unilateral-coverage}. Also, let 
    \begin{equation*}
        K=\Theta \left( \frac{S^2AB}{\epsilon}\log \left( \frac{S^2AB}{\delta}\right) \right)~.
    \end{equation*}
    Then, with probability at least $1-\delta$, F-PMVI with bonus term defined in \eqref{eq:filtering_bonus} outputs strategies $(\widehat{\pi},\widehat{\mu})$ with
    \begin{equation*}
        \optgap(\widehat{\pi},\widehat{\nu}) \leq O \left( H(H\sqrt{S}+\gamma)\sqrt{\epsilon} \right) ~.
    \end{equation*}
\end{thm}


    Note that there is no direct dependence of the bounds on $K$, and thus, it seems like, as $\epsilon$ approaches $0$, the estimated strategies converge to the NE equilibria. This is due to the constraint we put on  $K$. The filtering oracle assumes that the number of samples is large enough that the error coming from the sample mean estimation is dominated by the error coming from corruption, and thus, that term is omitted in the $O$ notation.  



% However, note that $\Phi$ in this case is the identity matrix, and thus the covariance matrix of the observations becomes diagonal. Thus, we ask the question:

% \textit{Given an arbitrary corruption model of offline data associated with a tabular MG, that satisfies unilateral coverage, can we improve the order of $H$ in the bounds, while maintaining optimal order of $\epsilon$?}


